A Framework for Visually Realistic Multi-robot Simulation in Natural Environment

This paper presents a generalized framework for the simulation of multiple robots and drones in highly realistic models of natural environments. The proposed simulation architecture uses the Unreal Engine4 for generating both optical and depth sensor outputs from any position and orientation within the environment and provides several key domain specific simulation capabilities. Various components and functionalities of the system have been discussed in detail. The simulation engine also allows users to test and validate a wide range of computer vision algorithms involving different drone configurations under many types of environmental effects such as wind gusts. The paper demonstrates the effectiveness of the system by giving experimental results for a test scenario where one drone tracks the simulated motion of another in a complex natural environment.

==> sim_approach.tex <==
\renewcommand{\labelitemi}{\ding{112}}
\begin{tikzpicture} 
   \tikzset{
     box/.style    = { rounded corners = 5pt,
                       align           = left,
                       font            = \sffamily\footnotesize,
                       text width      = 3.85cm, 
                       blur shadow     = {shadow blur steps = 15} },    
     legend/.style = { font       = \sffamily\bfseries, 
                       align      = right,
                       text width = 3.4cm},
  }
  \node [shade,
    blur shadow  = {shadow blur steps = 15},
    text width   = 1.01\textwidth,
    top color    = gray, 
    bottom color = white,
    text         = black, 
    font         = \sffamily\bfseries\large] (A)
    {Simulation Tools\\ \vspace{.6\textwidth} 
    ..};
  
  \node [box, below left  = -4.5cm and -3.85cm of A, fill = YellowGreen]
    (DE)
    {\underline{\bfseries Discrete Event (DE)}
      \begin{itemize} 
        \setlength{\itemindent} {-.5cm}
        \item entities (passive objects)
        \item flowcharts 
        \item network ressources
      \end{itemize}
    };

  \node [box, above right  = -3.5cm and .5cm of DE,
    minimum height=0.55\textwidth, fill = YellowGreen, text depth = 0.35\textwidth]
    (AB)
    { \underline{\bfseries Agent Based (AB)} 
        \begin{itemize} \setlength{\itemindent}{-.5cm}
          \item Active objects
          \item Individual behavior rules
          \item (In)direct interaction
          \item Environnement models
          \end{itemize}  
    };

  \node [box, above right  = -2.cm and .5cm of AB, fill = YellowGreen]
    (SD)
    { \underline{\bfseries System Dynamics (SD)}
      \begin{itemize} \setlength{\itemindent}{-.5cm}
        \item Levels (aggregates)
        \item Stocks \& flow diagrams
        \item Feedback loops
      \end{itemize}
    };

  \node [legend, above left = -1.25cm and 4.75cm of AB] (HA)
    {High Abstraction \\ Less Details \\ Macro Level};

  \node [legend, below = 1.5cm of HA] (MA)
    {Middle Abstraction \\ Average Details \\ Meso Level};
  
  \node [legend, below = 1.5cm of MA] (LA)
    {Low Abstraction \\ More Details \\ Micro Level};

  \node [below = 1.25cm of AB, font = \sffamily\bfseries\large ] (d1) 
    {Mostly Single threaded $\triangleleft$};

  \node [right = .5cm of d1, font = \sffamily\bfseries\large ] (d2) 
    {$\triangleright$ Usually distributed };
  
   %\path [ draw, color = Gray, dashed, line width = 2pt ]
   %  (d1.south east) + (0.3cm,0)   coordinate(x1) -- (x1|-A.north);  
   
   \path [draw, ->, >=latex, line width = 2pt ]
     (A.south west)  + (-0.25cm,0) coordinate(x2) -- (x2|-A.north);
\end{tikzpicture}
